The LLM Language Network: A Neuroscientific Approach for Identifying Causally Task-Relevant Units

Large language models (LLMs) exhibit remarkable capabilities on not just language tasks, but also various tasks that are not linguistic in nature, such as logical reasoning and social inference. In the human brain, neuroscience has identified a core language system that selectively and causally supports language processing. We here ask whether similar specialization for language emerges in LLMs. We identify language-selective units within 18 popular LLMs, using the same localization approach that is used in neuroscience. We then establish the causal role of these units by demonstrating that ablating LLM language-selective units -- but not random units -- leads to drastic deficits in language tasks. Correspondingly, language-selective LLM units are more aligned to brain recordings from the human language system than random units. Finally, we investigate whether our localization method extends to other cognitive domains: while we find specialized networks in some LLMs for reasoning and social capabilities, there are substantial differences among models. These findings provide functional and causal evidence for specialization in large language models, and highlight parallels with the functional organization in the brain.

==> tables/models.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

\begin{table}[ht]
\centering
\begin{tabular}{@{}llcc@{}}
\toprule
& \textbf{Model}           & \multicolumn{1}{l}{\textbf{Lang}} & \multicolumn{1}{l}{\textbf{MD/ToM}}  \\ \midrule
   & GPT2-Large               & \cmark                                    & \xmark           \\
   & GPT2-XL                  & \cmark                                    & \xmark            \\
   & Gemma-2B                 & \cmark                                    & \xmark             \\
   & Gemma-7B                 & \cmark                                    & \xmark             \\
   & Gemma-1.1-7B-Instruct    & \xmark                                    & \cmark              \\
   & Phi-3.5-Mini-Instruct    & \cmark                                    & \cmark              \\
   & Mistral-7B-v0.3          & \cmark                                    & \xmark             \\
   & Mistral-7B-Instruct-v0.3 & \xmark                                    & \cmark              \\
   & LLaMA-2-7B               & \cmark                                    & \xmark             \\
   & LLaMA-2-7B-Chat          & \xmark                                    & \cmark              \\
   & LLaMA-2-13B              & \cmark                                    & \xmark             \\
   & LLaMA-2-13B-Chat         & \xmark                                    & \cmark              \\       
   & LLaMA-3.1-8B-Instruct    & \cmark                                    & \cmark              \\
   & LLaMA-3.2-3B-Instruct    & \xmark                                    & \cmark              \\
   & Falcon-7B                & \cmark                                    & \xmark             \\
   & Falcon-7B-Instruct       & \xmark                                    & \cmark              \\
   & Qwen2.5-3B-Instruct      & \xmark                                    & \cmark              \\
   & Qwen2.5-7B-Instruct      & \xmark                                    & \cmark              \\ \midrule
 \textbf{\#}         & 18   & 10                                    & 10                      
\\ \bottomrule
\end{tabular}
\caption{
  \textbf{Models used in this work}
  Overview of the 18 models analyzed, with an indication of the specific experiments in which each model was used. Lang referes to the language experiments, MD refers to the multiple demand experiments, and ToM refers to the theory of mind experiments.
}
\label{tab:models}
\end{table}
